Learning with Confident Examples: Rank Pruning for Robust Classification with Noisy Labels

Noisy PN learning is the problem of binary classification when training examples may be mislabeled (flipped) uniformly with noise rate rho1 for positive examples and rho0 for negative examples. We propose Rank Pruning (RP) to solve noisy PN learning and the open problem of estimating the noise rates, i.e. the fraction of wrong positive and negative labels. Unlike prior solutions, RP is time-efficient and general, requiring O(T) for any unrestricted choice of probabilistic classifier with T fitting time. We prove RP has consistent noise estimation and equivalent expected risk as learning with uncorrupted labels in ideal conditions, and derive closed-form solutions when conditions are non-ideal. RP achieves state-of-the-art noise estimation and F1, error, and AUC-PR for both MNIST and CIFAR datasets, regardless of the amount of noise and performs similarly impressively when a large portion of training examples are noise drawn from a third distribution. To highlight, RP with a CNN classifier can predict if an MNIST digit is a "one"or "not" with only 0.25% error, and 0.46 error across all digits, even when 50% of positive examples are mislabeled and 50% of observed positive labels are mislabeled negative examples.

==> uai_rp_arxiv copy/0_conclusion.tex <==
\section{Discussion}

To our knowledge, Rank Pruning is the first time-efficient algorithm, w.r.t. classifier fitting time, for $\tilde{P}\tilde{N}$ learning that achieves similar or better F1, error, and AUC-PR than current state-of-the-art methods across practical scenarios for synthetic, MNIST, and CIFAR datasets, with logistic regression and CNN classifiers, across all noise rates, $\rho_1, \rho_0$, for varying added noise, dimension, separability, and number of training examples. By \emph{learning with confident examples}, we discover provably consistent estimators for noise rates, $\rho_1$, $\rho_0$, derive theoretical solutions when $g$ is unassuming, and accurately uncover the classifications of $f$ fit to hidden labels, perfectly when $g$ range separates $P$ and $N$.

We recognize that disambiguating whether we are in the unassuming or range separability condition may be desirable. Although knowing $g^*(x)$ and thus $\Delta g(x)$ is impossible, if we assume randomly uniform noise, and toggling the $LB_{y=1}$ threshold does not change $\rho^{conf}_1$, then $g$ range separates $P$ and $N$. When $g$ is unassuming, Rank Pruning is still robust to imperfect $g(x)$ within a range separable subset of $P$ and $N$ by training with confident examples even when noise rate estimates are inexact.

An important contribution of Rank Pruning is generality, both in classifier and implementation. The use of logistic regression and a generic CNN in our experiments emphasizes that our findings are not dependent on model complexity. We evaluate thousands of scenarios to avoid findings that are an artifact of problem setup. A key point of Rank Pruning is that we only report the simplest, non-parametric version. For example, we use 3-fold cross-validation to compute $g(x)$ even though we achieved improved performance with larger folds. We tried many variants of pruning and achieved significant higher F1 for MNIST and CIFAR, but to maintain generality, we present only the basic model.

At its core, Rank Pruning is a simple, robust, and general solution for noisy binary classification by \emph{learning with confident examples}, but it also challenges how we think about training data. For example, SVM showed how a decision boundary can be recovered from only support vectors. Yet, when training data contains significant mislabeling, confident examples, many of which are far from the boundary, are informative for uncovering the true relationship $P(y=1|x)$. Although modern affordances of ``big data" emphasize the value of \emph{more} examples for training, through Rank Pruning we instead encourage a rethinking of learning with \emph{confident} examples.

% Inspired by modern affordances, ``big data" in statistical learning has emphasized the value of \emph{more} examples for training. In the way that SVM changed the way we think about training examples by showing how a boundary condition can be recovered using only support vectors, through Rank Pruning we encourage a deeper understanding of the value of training with \emph{confident} examples.

% Although we emphasize theoretical justification for Rank Pruning, it is important to emphasize three high level ideas it embodies. First, we select confident examples that will remain, and prune the rest, based on ranking, not exact probability. When data is prone to mislabeling, top-ranked candidates , an inherently simpler problem to solve than exact probablity estimation. Although  choice to use pruning is motivated by Pruning instead of flipping because (1) removes noise, (2) little difference in practice, (3) easier to analyze, (4) less penalty for removing a correctly labeled 

% Emphasize how well we do in teh cases of extreme noise.


% An additional contribution of this paper is that we prove the improvement of our method when (1) the classifier is imperfect and perfect, whereas all literature that we are aware of focuses on perfect classification, and (2) to our knowledge, we are the first paper to theoretically evaluation and use our best sample adaptation method.

% our work extends to semi-supervised learning. Just add unlabeled examples as s = 0.

% OLD NOTES FROM ORIGINAL PAPER (remove unsupported claims, don't be too bold):

% The current belief in machine learning and big data is that more data for training is better. Iterative Pruning shifts this paradigm to suggest the benefits of instead focus on, not more data, but the best data.

% The methodology we've presented is quite powerful. It is trivial to implement, interpretable even for novices, robust to input noise and mislabeling, and produces more accurate results than any prior method. Summarize summarize summarize

% 1. Simplicity of iterative pruning
% 3. Markedly significant improvement above state-of-the-art in all categories.


% We remind the reader of the Free-Lunch Theorem which states that any two optimization algorithms are equivalent when their performance is averaged across all possible problems. Then, how does Iterative Pruning seemingly perform so well when compared with prior state-of-the-art? Iterative Pruning ``circumvents the lunch line" by pruning out the ``bad problems." When training examples have poor discrimination, high noise, or are mislabeled, Iterative Pruning tries to remove these bad examples, instead training on likely good examples, seeking examples for which it can predict their label with high probability. This ideology is more general than PU learning.

% Although we only consider Iterative Pruning within the context of PU learning, the ``only train on good examples" ideology is generalizable to supervised and semi-supervised classification. For example, our analysis of Iterative Pruning in the presence of mislabeled positive examples can be re-framed as an algorithm for semi-supervised learning, since both the labeled and unlabeled sets have. In the Iterative Pruning case, we make assumptions about our input (that the labeled set is more likely to contain positives and the unlabeled set is more likely to contain negatives).

% \subsection{Contributions}

% Unlike prior work, both Part 1 and Part 2 of Algorithm 1 are computationally efficient and can be used with any binary probabilistic estimator (i.e. classifier) and we provide exact theoretical estimation allowing for imperfect probability estimation and overlapping $P$ and $N$ distributions. This includes the case when imperfect probability estimation is due to added noise drawn from a third distribution. We evaluate our algorithm on the MNIST and CIFAR datasets, achieving state-of-the-art estimation of $\rho_1$ and $\rho_0$, state-of-the-art performance across F1, AUC, and Error metrics, and consistent theoretical and empirical results, regardless of $\rho_1$ and $\rho_0$.

==> uai_rp_arxiv copy/0_experimental.tex <==

\section{Experimental Results}
\label{sec:experimental}




In Section \ref{methodology}, we developed a theoretical framework for Rank Pruning, proved exact noise estimation and equivalent expected risk when conditions are ideal, and derived closed-form solutions when conditions are non-ideal. Our theory suggests that, in practice, Rank Pruning should (1) accurately estimate $\rho_1$ and $\rho_0$, (2) typically achieve as good or better F1, error and AUC-PR \citep{Davis:2006:RPR:1143844.1143874} as state-of-the-art methods, and (3) be robust to both mislabeling and added noise. 

In this section, we support these claims with an evaluation of the comparative performance of Rank Pruning in non-ideal conditions across thousands of scenarios. These include less complex (MNIST) and more complex (CIFAR) datasets,  simple (logistic regression) and complex (CNN) classifiers, the range of noise rates, added random noise, separability of $P$ and $N$, input dimension, and number of training examples to ensure that Rank Pruning is a general, agnostic solution for $\tilde{P}\tilde{N}$ learning.

\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{synthetic_F1_horizontal.pdf}}
\caption{Comparison of Rank Pruning with different noise ratios $(\pi_1, \rho_1)$ on a synthetic dataset for varying separability $d$, dimension, added random noise and number of training examples. Default settings for Fig. \ref{synthetic_F1}, \ref{synthetic_diff_tp} and \ref{synthetic_comparison}: $d=4$, 2-dimension, $0\%$ random noise, and 5000 training examples with $p_{y1}=0.2$. The lines are an average of 200 trials.}
\label{synthetic_F1}
\end{center}
\vskip -0.3in
\end{figure}

\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=0.75\columnwidth]{synthetic_diff_tp_horizontal.pdf}}
\caption{Sum of absolute difference between theoretically estimated $\hat{\rho}_i^{thry}$ and empirical $\hat{\rho}_i$, $i=0,1$, with five different $(\pi_1, \rho_1)$, for varying separability $d$, dimension, and number of training examples. Note that no figure exists for percent random noise because the theoretical estimates in Eq. (\ref{rho_imperfect_condition}) do not address added noise examples.}
\label{synthetic_diff_tp}
\end{center}
\vskip -0.3in
\end{figure}


In our experiments, we adjust $\pi_1$ instead of $\rho_0$ because binary noisy classification problems (e.g. detection and recognition tasks) often have that $|P| \ll |N|$. This choice allows us to adjust both noise rates with respect to $P$, i.e. the fraction of true positive examples that are mislabeled as negative ($\rho_1$) and the fraction of observed positive labels that are actually mislabeled negative examples ($\pi_1$). The $\tilde{P}\tilde{N}$ learning algorithms are trained with corrupted labels $s$, and tested on an unseen test set by comparing predictions $\hat{y}$ with the true test labels $y$ using F1 score, error, and AUC-PR metrics. We include all three to emphasize our apathy toward tuning results to any single metric. We provide F1 scores in this section with error and AUC-PR scores in Appendix \ref{sec:tables_appendix}.

\subsection{Synthetic Dataset}
The synthetic dataset is comprised of a Guassian positive class and a Guassian negative classes such that negative examples ($y=0$) obey an $m$-dimensional Gaussian distribution $N(\mathbf{0}, \mathbf{I})$ with unit variance $\mathbf{I}=diag(1,1,...1)$, and positive examples obey $N(d\mathbf{1}, 0.8\mathbf{I})$, where $d\mathbf{1}=(d,d,...d)$ is an $m$-dimensional vector, and $d$ measures the separability of the positive and negative set.

We test Rank Pruning by varying 4 different settings of the environment: separability $d$, dimension, number of training examples $n$, and percent (of $n$) added random noise drawn from a uniform distribution $U([-10,10]^m)$. In each scenario, we test 5 different $(\pi_1,\rho_1)$ pairs: $(\pi_1,\rho_1)\in\{(0,0),(0,0.5),(0.25,0.25)$, $(0.5,0),(0.5,0.5)\}$. From Fig. \ref{synthetic_F1}, we observe that across these settings, the F1 score for Rank Pruning is fairly agnostic to magnitude of mislabeling (noise rates). As a validation step, in Fig. \ref{synthetic_diff_tp} we measure how closely our empirical estimates match our theoretical solutions in Eq. (\ref{rho_imperfect_condition}) and find near equivalence except when the number of training examples approaches zero.

For significant mislabeling ($\rho_1=0.5$, $\pi_1=0.5$), Rank Pruning often outperforms other methods (Fig. \ref{synthetic_comparison}). In the scenario of different separability $d$, it achieves nearly the same F1 score as the ground truth classifier. Remarkably, from Fig. \ref{synthetic_F1} and Fig. \ref{synthetic_comparison}, we observe that when added random noise comprises $50\%$ of total training examples, Rank Pruning still achieves F1 $>$ 0.85, compared with F1 $<$ 0.5 for all other methods. This emphasizes a unique feature of Rank Pruning, it will also remove added random noise because noise drawn from a third distribution is unlikely to appear confidently positive or negative.


\subsection{MNIST and CIFAR Datasets}


We consider the binary classification tasks of one-vs-rest for the MNIST \citep{lecun-mnisthandwrittendigit-2010} and CIFAR-10 (\cite{cifar10}) datasets, e.g. the ``car vs rest" task in CIFAR is to predict if an image is a ``car" or ``not". $\rho_1$ and $\pi_1$ are given to all $\tilde{P}\tilde{N}$ learning methods for fair comparison, except for $RP_\rho$ which is Rank Pruning including noise rate estimation. $RP_\rho$ metrics measure our performance on the unadulterated $\tilde{P}\tilde{N}$ learning problem.



\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{synthetic_comparison_horizontal.pdf}}
\caption{Comparison of $\tilde{P}\tilde{N}$ methods for varying separability $d$, dimension, added random noise, and number of training examples for $\pi_1=0.5$, $\rho_1=0.5$ (given to all methods).
%The default parameters are: $d=4$, 2 dimensional input, $0\%$ random noise, and 5000 training examples with $p_{y1}=0.2$. Lines are an average of 200 trials.
}
\label{synthetic_comparison}
\end{center}
\vskip -0.15in
\end{figure}

\begin{figure}[b!]
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{rho1_pi1_heatmap_vs_true.pdf}}
\vskip -0.08in
\caption{Rank Pruning $\hat{\rho}_1$ and $\hat{\pi}_1$ estimation consistency, averaged over all digits in MNIST. \textbf{(a)} Color depicts $\hat{\rho}_1-\rho_1$ with $\hat{\rho}_1$ (upper) and theoretical $\hat{\rho}_1^{thry}$ (lower) in each block. \textbf{(b)} Color depicts $\hat{\pi}_1-\pi_1$ with $\hat{\pi}_1$ (upper) and $\hat{\pi}_1^{thry}$ (lower) in each block. }
\label{rho1_pi1_mnist_logreg}
\end{center}
\vskip -0.1in
\end{figure} 

As evidence that Rank Pruning is dataset and classifier agnostic, we demonstrate its superiority with both (1) a linear logistic regression model with unit L2 regularization and (2) an AlexNet CNN variant with max pooling and dropout, modified to have a two-class output. The CNN structure is adapted from \cite{mnist_cnn_structure} for MNIST and \cite{cifar_cnn_structure} for CIFAR. CNN training ends when a 10\% holdout set shows no loss decrease for 10 epochs (max 50 for MNIST and 150 for CIFAR).

We consider noise rates \begin{small}{$\pi_1, \rho_1\in\{(0, 0.5),(0.25,0.25),$
$(0.5,0),(0.5,0.5)\}$}\end{small} for both MNIST and CIFAR, with additional settings for MNIST in Table \ref{table:mnist_cifar_logreg_f1} to emphasize Rank Pruning performance is noise rate agnostic. The $\rho_1=0$, $\pi_1=0$ case is omitted because when given $\rho_1$, $\pi_1$, all methods have the same loss function as the ground truth classifier, resulting in nearly identical F1 scores. Note that in general, Rank Pruning does not require perfect probability estimation to achieve perfect F1-score. As an example, this occurs when $P$ and $N$ are range-separable, and the rank order of the sorted $g(x)$ probabilities in $P$ and $N$ is consistent with the rank of the perfect probabilities, regardless of the actual values of $g(x)$.

For MNIST using logistic regression, we evaluate the consistency of our noise rate estimates with actual noise rates and theoretical estimates (Eq. \ref{rho_imperfect_condition}) across $\pi_1\in[0, 0.8] \times \rho_1\in[0,0.9]$. The computing time for one setting was $\sim10$ minutes on a single CPU core. The results for $\hat{\rho}_1$ and $\hat{\pi}_1$ (Fig. \ref{rho1_pi1_mnist_logreg}) are satisfyingly consistent, with mean absolute difference MD$_{\hat{\rho}_1, \rho_1}=0.105$ and  MD$_{\hat{\pi}_1, \pi_1}=0.062$, and validate our theoretical solutions (MD$_{\hat{\rho}_1,\hat{\rho}_1^{thry}}=0.0028$, MD$_{\hat{\pi}_1,\hat{\pi}_1^{thry}}=0.0058$). The deviation of the theoretical and empirical estimates reflects the assumption that we have infinite examples, whereas empirically, the number of examples is finite.



We emphasize two observations from our analysis on CIFAR and MNIST. First, Rank Pruning performs well in nearly every scenario and boasts the most dramatic improvement over prior state-of-the-art in the presence of extreme noise ($\pi_1=0.5$, $\rho_1=0.5$). This is easily observed in the right-most quadrant of Table \ref{table:mnist_cifar_cnn_f1}. The $\pi_1=0.5$, $\rho_1=0$ quadrant is nearest to $\pi_1=0$, $\rho_1=0$ and mostly captures CNN prediction variation because $|\tilde{P}| \ll |\tilde{N}|$.


Second, RP$_{\rho}$ often achieves equivalent (MNIST in Table \ref{table:mnist_cifar_cnn_f1}) or significantly higher (CIFAR in Tables \ref{table:mnist_cifar_logreg_f1} and \ref{table:mnist_cifar_cnn_f1}) F1 score than Rank Pruning when $\rho_1$ and $\pi_1$ are provided, particularly when noise rates are large. This effect is exacerbated for harder problems (lower F1 score for the ground truth classifier) like the ``cat” in CIFAR or the ``9” digit in MNIST likely because these problems are more complex, resulting in less confident predictions, and therefore more pruning. 

Remember that $\rho^{conf}_1$ and $\rho^{conf}_0$ are upper bounds when $g$ is unassuming. Noise rate overestimation accounts for the complexity of harder problems. As a downside, Rank Pruning may remove correctly labeled examples that ``confuse” the classifier, instead fitting only the confident examples in each class. We observe this on CIFAR in Table \ref{table:mnist_cifar_logreg_f1} where logistic regression severely underfits so that RP$_{\rho}$ has significantly higher F1 score than the ground truth classifier. Although Rank Pruning with noisy labels seemingly outperforms the ground truth model, if we lower the classification threshold to 0.3 instead of 0.5, the performance difference goes away by accounting for the lower probability predictions. 






\begin{table*}[t]

\setlength\tabcolsep{2pt} % Makes table columns tighter
\renewcommand{\arraystretch}{0.9}% Makes table rows tighter
\caption{Comparison of F1 score for one-vs-rest MNIST and CIFAR-10 (averaged over all digits/images) using logistic regression. Except for $RP_\rho$, $\rho_1$, $\rho_0$ are given to all methods. Top model scores are in bold with $RP_\rho$ in red if greater than non-RP models. Due to sensitivity to imperfect $g(x)$, \emph{Liu16} often
predicts the same label for all examples.
% in Tables \ref{table:mnist_cifar_logreg_f1} and \ref{table:mnist_cifar_cnn_f1}
%The $\pi_1=0$ quadrant in each dataset represents the "PU learning" case of $\tilde{P}\tilde{N}$ learning.
} 
\vskip -0.17in
\label{table:mnist_cifar_logreg_f1}
\begin{center}
\begin{small}
\begin{sc}


\resizebox{\textwidth}{!}{ %Completely zooms in or zooms out (shrinks) entire table!
\begin{tabular}{l|cccc|ccc|cccc|cccc|cccc}
\toprule

\multicolumn{0}{r|}{\textbf{Dataset}} & \multicolumn{4}{c|}{\textbf{CIFAR}} & \multicolumn{15}{c}{\textbf{MNIST}} \\

\multicolumn{0}{r|}{$\pi_1=$} & \textbf{0.0} & \textbf{0.25} & \textbf{0.5} & \textbf{0.5} &
\multicolumn{3}{c}{$\pi_1$\textbf{ = 0.0}}  &   
\multicolumn{4}{c}{$\pi_1$\textbf{ = 0.25}}  & 
\multicolumn{4}{c}{$\pi_1$\textbf{ = 0.5}}  & 
\multicolumn{4}{c}{$\pi_1$\textbf{ = 0.75}} 
\\

\textbf{Model,$\rho_1 = $} &   \textbf{0.5} &    \textbf{0.25} &    \textbf{0.0} &   \textbf{0.5} &  \textbf{0.25} &    \textbf{0.5} &   \textbf{0.75} &   \textbf{0.0} &    \textbf{0.25} &    \textbf{0.5} &   \textbf{0.75} &   \textbf{0.0} &    \textbf{0.25} &    \textbf{0.5} &   \textbf{0.75} &   \textbf{0.0} &    \textbf{0.25} &    \textbf{0.5} &   \textbf{0.75}    \\



\midrule

\textbf{True}   &  0.248 & 0.248 & 0.248 & 0.248 & 0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 &  0.894 \\
\textbf{RP}$_{\rho}$ &  \textcolor{red}{\textbf{0.301}}  & \textcolor{red}{\textbf{0.316}}  & \textcolor{red}{\textbf{0.308}}  & \textcolor{red}{\textbf{0.261}}  &  \textcolor{red}{\textbf{0.883}} &  \textcolor{red}{\textbf{0.874}} &  \textcolor{red}{\textbf{0.843}} &  \textcolor{red}{\textbf{0.881}} &  \textcolor{red}{\textbf{0.876}} &  \textcolor{red}{\textbf{0.863}} &  \textcolor{red}{\textbf{0.799}} &  0.823 &  0.831 &  \textcolor{red}{\textbf{0.819}} &  \textcolor{red}{\textbf{0.762}} &  0.583 &  0.603 &  0.587 &  0.532 \\
\textbf{RP} & \textbf{0.256} & \textbf{0.262} & \textbf{0.244} & 0.209 & \textbf{0.885} &  \textbf{0.873} &  \textbf{0.839} &  \textbf{0.890} &  \textbf{0.879} &  \textbf{0.863} &  \textbf{0.812} &  \textbf{0.879} &  \textbf{0.862} &  \textbf{0.838} &  \textbf{0.770} &  \textbf{0.855} &  \textbf{0.814} &  \textbf{0.766} &  0.617 \\
\textbf{Nat13} & 0.226 & 0.219 & 0.194 & 0.195 &  0.860 &  0.830 &  0.774 &  0.865 &  0.836 &  0.802 &  0.748 &  0.839 &  0.810 &  0.777 &  0.721 &  0.809 &  0.776 &  0.736 &  \textbf{0.640} \\
\textbf{Elk08} & 0.221  & 0.226  & 0.228  & \textbf{0.210}  &  0.862 &  0.830 &  0.771 &  0.864 &  0.847 &  0.819 &  0.762 &  0.843 &  0.835 &  0.814 &  0.736 &  0.674 &  0.669 &  0.599 &  0.473 \\
\textbf{Liu16} & 0.182 & 0.182 & 0.000 & 0.182 &   0.021 &  0.000 &  0.000 &  0.000 &  0.147 &  0.147 &  0.073 &  0.000 &  0.164 &  0.163 &  0.163 &  0.047 &  0.158 &  0.145 &  0.164 \\


\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


%%%% NEXT TABLE %%%%



\begin{table*}[t]

\setlength\tabcolsep{1pt} % Makes table columns tighter
\renewcommand{\arraystretch}{0.85}% Makes table rows tighter
\caption{F1 score comparison on MNIST and CIFAR-10 using a CNN. Except for $RP_\rho$, $\rho_1$, $\rho_0$ are given to all methods.
} 
\vskip -0.17in
\label{table:mnist_cifar_cnn_f1}
\begin{center}
\begin{small}
\begin{sc}

\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|ccccc|ccccc|ccccc|ccccc}
\toprule

\multicolumn{2}{l|}{\textbf{MNIST/CIFAR}} &  
% \multicolumn{1}{c|}{} & 
\multicolumn{5}{c|}{$\pi_1$\textbf{ = 0.0}}   &   
\multicolumn{5}{c|}{$\pi_1$\textbf{ = 0.25}}  & 
\multicolumn{10}{c}{$\pi_1$\textbf{ = 0.5}}   \\

\multicolumn{1}{l}{\textbf{IMAGE}} &  
\multicolumn{1}{c|}{} & 
% \multicolumn{5}{c}{$\rho_1$\textbf{ = 0}} & 
\multicolumn{5}{c|}{$\rho_1$\textbf{ = 0.5}} & 
\multicolumn{5}{c|}{$\rho_1$\textbf{ = 0.25}}  & 
\multicolumn{5}{c}{$\rho_1$\textbf{ = 0.0}} & 
\multicolumn{5}{c}{$\rho_1$\textbf{ = 0.5}}    \\

{\textbf{CLASS}} &   \textbf{True} & \textbf{RP}$_{\rho}$ &    \textbf{RP} & \textbf{Nat13} & \textbf{Elk08} & \textbf{Liu16} & \textbf{RP}$_{\rho}$ &    \textbf{RP} & \textbf{Nat13} & \textbf{Elk08} & \textbf{Liu16} & \textbf{RP}$_{\rho}$ &    \textbf{RP} & \textbf{Nat13} & \textbf{Elk08} & \textbf{Liu16} & \textbf{RP}$_{\rho}$ &    \textbf{RP} & \textbf{Nat13} & \textbf{Elk08} & \textbf{Liu16} \\
\midrule
\textbf{0}     &  0.993 &  \textcolor{red}{\textbf{0.991}} &  \textbf{0.988} &  0.977 &  0.976 &  0.179 &  \textcolor{red}{\textbf{0.991}} &  \textbf{0.992} &  0.982 &  0.981 &  0.179 &  \textcolor{red}{\textbf{0.991}} &  \textbf{0.992} &  0.984 &  0.987 &  0.985 &  \textcolor{red}{\textbf{0.989}} &  \textbf{0.989} &  0.937 &  0.964 &  0.179 \\
\textbf{1}     &  0.993 &  \textcolor{red}{\textbf{0.990}} &  \textbf{0.991} &  0.989 &  0.985 &  0.204 &  \textcolor{red}{\textbf{0.992}} &  \textbf{0.992} &  0.984 &  0.987 &  0.204 &  0.990 &  0.991 &  0.992 &  \textbf{0.993} &  0.990 &  \textcolor{red}{\textbf{0.989}} &  \textbf{0.989} &  0.984 &  0.988 &  0.204 \\
\textbf{2}     &  0.987 &  \textcolor{red}{\textbf{0.973}} &  \textbf{0.976} &  0.972 &  0.969 &  0.187 &  \textcolor{red}{\textbf{0.984}} &  \textbf{0.983} &  0.978 &  0.975 &  0.187 &  0.985 &  0.986 &  0.985 &  0.986 &  \textbf{0.988} &  \textcolor{red}{\textbf{0.971}} &  \textbf{0.975} &  0.968 &  0.959 &  0.187 \\
\textbf{3}     &  0.990 &  \textcolor{red}{\textbf{0.984}} &  \textbf{0.984} &  0.972 &  0.981 &  0.183 &  \textcolor{red}{\textbf{0.986}} &  \textbf{0.986} &  0.978 &  0.978 &  0.183 &  \textcolor{red}{\textbf{0.990}} &  0.987 &  \textbf{0.989} &  \textbf{0.989} &  0.984 &  \textcolor{red}{\textbf{0.981}} &  \textbf{0.979} &  0.957 &  0.971 &  0.183 \\
\textbf{4}     &  0.994 &  \textcolor{red}{\textbf{0.981}} &  0.979 &  \textbf{0.981} &  0.977 &  0.179 &  \textcolor{red}{\textbf{0.985}} &  \textbf{0.987} &  0.971 &  0.964 &  0.179 &  0.987 &  \textbf{0.990} &  \textbf{0.990} &  0.989 &  0.985 &  \textcolor{red}{\textbf{0.977}} &  \textbf{0.982} &  0.955 &  0.961 &  0.179 \\
\textbf{5}     &  0.989 &  \textcolor{red}{\textbf{0.982}} &  \textbf{0.980} &  0.978 &  0.979 &  0.164 &  \textcolor{red}{\textbf{0.985}} &  \textbf{0.982} &  0.964 &  0.965 &  0.164 &  \textcolor{red}{\textbf{0.988}} &  \textbf{0.987} &  \textbf{0.987} &  0.984 &  \textbf{0.987} &  \textcolor{red}{\textbf{0.965}} &  \textbf{0.968} &  0.962 &  0.957 &  0.164 \\
\textbf{6}     &  0.989 &  \textcolor{red}{\textbf{0.986}} &  \textbf{0.985} &  0.972 &  0.982 &  0.175 &  \textcolor{red}{\textbf{0.985}} &  \textbf{0.987} &  0.978 &  0.981 &  0.175 &  0.985 &  0.985 &  \textbf{0.988} &  0.987 &  0.985 &  \textcolor{red}{\textbf{0.983}} &  \textbf{0.982} &  0.946 &  0.959 &  0.175 \\
\textbf{7}     &  0.987 &  \textcolor{red}{\textbf{0.981}} &  \textbf{0.980} &  0.967 &  0.948 &  0.186 &  \textcolor{red}{\textbf{0.976}} &  \textbf{0.975} &  0.971 &  0.971 &  0.186 &  0.976 &  0.980 &  \textbf{0.985} &  0.982 &  0.983 &  \textcolor{red}{\textbf{0.973}} &  \textbf{0.968} &  0.942 &  0.958 &  0.186 \\
\textbf{8}     &  0.989 &  \textcolor{red}{\textbf{0.975}} &  \textbf{0.978} &  0.943 &  0.967 &  0.178 &  \textcolor{red}{\textbf{0.982}} &  \textbf{0.981} &  0.967 &  0.951 &  0.178 &  0.982 &  \textbf{0.984} &  0.982 &  0.979 &  0.983 &  \textcolor{red}{\textbf{0.977}} &  \textbf{0.975} &  0.864 &  0.959 &  0.178 \\
\textbf{9}     &  0.982 &  0.966 &  \textbf{0.974} &  0.972 &  0.935 &  0.183 &  \textcolor{red}{\textbf{0.976}} &  \textbf{0.974} &  0.967 &  0.967 &  0.183 &  0.976 &  0.975 &  0.974 &  \textbf{0.978} &  0.970 &  \textcolor{red}{\textbf{0.959}} &  0.940 &  0.931 &  \textbf{0.942} &  0.183 \\
\midrule
\textbf{AVG$_{MN}$} &  0.989 &  \textcolor{red}{\textbf{0.981}} &  \textbf{0.981} &  0.972 &  0.970 &  0.182 &  \textcolor{red}{\textbf{0.984}} &  \textbf{0.984} &  0.974 &  0.972 &  0.182 &  0.985 &  \textbf{0.986} &  \textbf{0.986} &  0.985 &  0.984 &  \textcolor{red}{\textbf{0.976}} &  \textbf{0.975} &  0.945 &  0.962 &  0.182 \\


\midrule

\textbf{plane}   &  0.755 &  \textcolor{red}{\textbf{0.689}} &  \textbf{0.634} &  0.619 &  0.585 &  0.182 &  \textcolor{red}{\textbf{0.695}} &  \textbf{0.702} &  0.671 &  0.640 &  0.182 &  \textcolor{red}{\textbf{0.757}} &  \textbf{0.746} &  0.716 &  0.735 &    0.000 &  \textcolor{red}{\textbf{0.628}} &  \textbf{0.635} &  0.459 &  0.598 &  0.182 \\
\textbf{auto} &  0.891 &  \textcolor{red}{\textbf{0.791}} &  \textbf{0.785} &  0.761 &  0.768 &  0.000 &  \textcolor{red}{\textbf{0.832}} &  \textbf{0.824} &  0.771 &  0.783 &  0.182 &  0.862 &  0.866 &  \textbf{0.869} &  0.865 &    0.000 &  \textcolor{red}{\textbf{0.749}} &  \textbf{0.720} &  0.582 &  0.501 &  0.182 \\
\textbf{bird}       &  0.669 &  \textcolor{red}{\textbf{0.504}} &  \textbf{0.483} &  0.445 &  0.389 &  0.182 &  \textcolor{red}{\textbf{0.543}} &  \textbf{0.515} &  0.469 &  0.426 &  0.182 &  \textcolor{red}{\textbf{0.577}} &  \textbf{0.619} &  0.543 &  0.551 &    0.000 &  \textcolor{red}{\textbf{0.447}} &  \textbf{0.409} &  0.366 &  0.387 &  0.182 \\
\textbf{cat}        &  0.487 &  \textcolor{red}{\textbf{0.350}} &  0.279 &  0.310 &  \textbf{0.313} &  0.000 &  \textcolor{red}{\textbf{0.426}} &  0.317 &  \textbf{0.350} &  0.345 &  0.182 &  \textcolor{red}{\textbf{0.489}} &  \textbf{0.433} &  0.426 &  0.347 &    0.000 &  \textcolor{red}{\textbf{0.394}} &  0.282 &  0.240 &  \textbf{0.313} &  0.182 \\
\textbf{deer}       &  0.726 &  \textcolor{red}{\textbf{0.593}} &  \textbf{0.540} &  0.455 &  0.522 &  0.182 &  \textcolor{red}{\textbf{0.585}} &  0.554 &  0.480 &  \textbf{0.569} &  0.182 &  0.614 &  0.630 &  \textbf{0.643} &  0.633 &    0.000 &  \textcolor{red}{\textbf{0.458}} &  0.375 &  0.310 &  \textbf{0.383} &  0.182 \\
\textbf{dog}        &  0.569 &  \textcolor{red}{\textbf{0.544}} &  \textbf{0.577} &  0.429 &  0.456 &  0.000 &  \textcolor{red}{\textbf{0.579}} &  0.559 &  0.569 &  \textbf{0.576} &  0.182 &  0.647 &  0.637 &  \textbf{0.667} &  0.630 &    0.000 &  \textcolor{red}{\textbf{0.516}} &  0.461 &  0.412 &  \textbf{0.465} &  0.182 \\
\textbf{frog}       &  0.815 &  \textcolor{red}{\textbf{0.746}} &  0.727 &  \textbf{0.733} &  0.718 &  0.000 &  \textcolor{red}{\textbf{0.729}} &  \textbf{0.750} &  0.630 &  0.584 &  0.182 &  0.767 &  \textbf{0.782} &  0.777 &  0.770 &    0.000 &  \textcolor{red}{\textbf{0.635}} &  \textbf{0.615} &  0.589 &  0.524 &  0.182 \\
\textbf{horse}      &  0.805 &  \textcolor{red}{\textbf{0.690}} &  0.670 &  0.624 &  \textbf{0.672} &  0.182 &  \textcolor{red}{\textbf{0.710}} &  0.669 &  \textbf{0.683} &  0.627 &  0.182 &  0.761 &  \textbf{0.776} &  0.769 &  0.753 &    0.000 &  \textcolor{red}{\textbf{0.672}} &  \textbf{0.569} &  0.551 &  0.461 &  0.182 \\
\textbf{ship}       &  0.851 &  \textcolor{red}{\textbf{0.791}} &  \textbf{0.783} &  0.719 &  0.758 &  0.182 &  \textcolor{red}{\textbf{0.810}} &  \textbf{0.801} &  0.758 &  0.723 &  0.182 &  0.816 &  0.822 &  0.830 &  \textbf{0.831} &    0.000 &  \textcolor{red}{\textbf{0.715}} &  \textbf{0.738} &  0.569 &  0.632 &  0.182 \\
\textbf{truck}      &  0.861 &  \textcolor{red}{\textbf{0.744}} &  \textbf{0.722} &  0.655 &  0.665 &  0.182 &  \textcolor{red}{\textbf{0.814}} &  \textbf{0.826} &  0.798 &  0.774 &  0.182 &  0.812 &  0.830 &  \textbf{0.826} &  0.824 &    0.000 &  \textcolor{red}{\textbf{0.654}} &  0.543 &  0.575 &  \textbf{0.584} &  0.182 \\
\midrule
\textbf{AVG$_{CF}$}      &  0.743 &  \textcolor{red}{\textbf{0.644}} &  \textbf{0.620} &  0.575 &  0.585 &  0.109 &  \textcolor{red}{\textbf{0.672}} &  \textbf{0.652} &  0.618 &  0.605 &  0.182 &  \textcolor{red}{\textbf{0.710}} &  \textbf{0.714} &  0.707 &  0.694 &    0.000 &  \textcolor{red}{\textbf{0.587}} &  \textbf{0.535} &  0.465 &  0.485 &  0.182 \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> uai_rp_arxiv copy/0_framing.tex <==

\section{Framing the \texorpdfstring{$\tilde{P}\tilde{N}$}{Noisy PN} Learning Problem }
\label{sec:framing}

\vskip -0.04in

In this section, we formalize the foundational definitions, assumptions, and goals of the $\tilde{P}\tilde{N}$ learning problem illustrated by the student-teacher motivational example.

Given $n$ observed training examples $x \in \mathcal{R}^D$ with associated observed corrupted labels $s \in \{0,1\}$ and unobserved true labels $y \in \{0,1\}$, we seek a binary classifier $f$ that estimates the mapping $x\to y$. Unfortunately, if we fit the classifier using observed $(x, s)$ pairs, we estimate the mapping $x\to s$ and obtain $g(x)=P(\hat{s}=1|x)$. 

We define the observed noisy positive and negative sets as $\tilde{P} = \{x| s = 1\}, \tilde{N} = \{x| s = 0\}$ and the unobserved true positive and negative sets as $P = \{x| y = 1\}, N = \{x| y = 0\}$. Define the hidden training data as $D=\{(x_1, y_1), (x_2, y_2), ..., (x_n, y_n)\}$, drawn i.i.d. from some true distribution $\mathcal{D}$. 
% We assume that a class-conditional extension of the Classification Noise Process (CNP) \citep{angluin1988learning} maps $y$ true labels to $s$ observed labels such that each label in $P$ is flipped independently with probability $\rho_1$ and each label in $N$ is flipped independently with probability $\rho_0$ ($s \leftarrow CNP(y, \rho_1, \rho_0)$). 
We assume that a class-conditional Classification Noise Process (CNP) \citep{angluin1988learning} maps $y$ true labels to $s$ observed labels such that each label in $P$ is flipped independently with probability $\rho_1$ and each label in $N$ is flipped independently with probability $\rho_0$ ($s \leftarrow CNP(y, \rho_1, \rho_0)$). 
The resulting observed, corrupted dataset is $D_{\rho}=\{(x_1, s_1), (x_2, s_2), ..., (x_n, s_n)\}$. Therefore, $(s \independent x) | y$ and $P(s=s|y=y,x) = P(s=s|y=y)$. In recent work, CNP is referred to as the random noise classification (RCN) noise model \citep{Liu:2016:CNL:2914183.2914328, NIPS2013_5073}.

The noise rate $\rho_1 = P(s=0|y=1)$ is the fraction of $P$ examples mislabeled as negative and the noise rate $\rho_0 = P(s=1|y=0)$ is the fraction of $N$ examples mislabeled as positive. Note that $\rho_1 + \rho_0 < 1$ is a necessary condition, otherwise more examples would be mislabeled than labeled correctly. Thus, $\rho_0 < 1- \rho_1$. We elect a subscript of ``0" to refer to the negative set and a subscript of ``1" to refer to the positive set. Additionally, let $p_{s1} = P(s=1)$ be the fraction of corrupted labels that are positive and  $p_{y1} = P(y=1)$ be the fraction of true labels that are positive. It follows that the inversed noise rates are $\pi_1 = P(y=0|s=1) =  \frac{\rho_0 (1 - p_{y1})}{p_{s1}}$ and $\pi_0 = P(y=1|s=0) =  \frac{\rho_1 p_{y1}}{(1 - p_{s1})}$. Combining these relations, given any pair in $\{(\rho_0, \rho_1),(\rho_1, \pi_1),(\rho_0, \pi_0), (\pi_0, \pi_1)\}$, the remaining two and $p_{y1}$ are known. %The meaning of each noise rate is summarized in Table \ref{}. 

We consider five levels of assumptions for $P$, $N$, and $g$: \\
\textbf{Perfect Condition}: $g$ is a ``perfect" probability estimator iff $g(x) = g^*(x)$ where $g^*(x) = P(s=1|x)$. Equivalently, let $g(x) = P(s=1|x)+\Delta g(x)$. Then $g(x)$ is ``perfect" when $\Delta g(x) = 0$ and ``imperfect" when $\Delta g(x) \neq 0$. $g$ may be imperfect due to the method of estimation or due to added uniformly randomly labeled examples drawn from a third noise distribution.\\
\textbf{Non-overlapping Condition}: $P$ and $N$ have ``non-overlapping support" if $P(y=1|x) = \indicator{y=1}$, where the indicator function $\indicator{a}$ is $1$ if the $a$ is true, else $0$. \\
\textbf{Ideal Condition}\footnote{ Eq. (\ref{eq1}) is first derived in \citep{Elkan:2008:LCO:1401890.1401920} .}: $g$ is ``ideal" when both perfect and non-overlapping conditions hold and $(s \independent x) | y$ such that


\vskip -0.25in
\begin{equation} \label{eq1}
\begin{split}
g(x) = & g^*(x) = P(s=1|x) \\ 
 = & P(s=1|y=1,x) \cdot P(y=1|x) + P(s=1|y=0,x) \cdot P(y=0|x) \\
 = & (1 - \rho_1) \cdot \mathbbm{1}[[y=1]] + \rho_0 \cdot \mathbbm{1}[[y=0]]
\end{split}
\end{equation}
\vskip -0.1in

\textbf{Range Separability Condition} $g$ range separates $P$ and $N$ iff $\forall x_1\in P$ and $\forall x_2 \in N$, we have $g(x_1) >g(x_2)$. \\
\textbf{Unassuming Condition}: $g$ is ``unassuming" when perfect and/or non-overlapping conditions may not be true. 

Their relationship is:
$\textbf{Unassuming}\supset\textbf{Range}$ $\textbf{Separability}$ $\supset\textbf{Ideal}=\textbf{Perfect}\cap\textbf{Non-overlapping}$. 

We can now state the two goals of Rank Pruning for $\tilde{P}\tilde{N}$ learning. \textbf{Goal 1} is to perfectly estimate $\hat{\rho}_1 \estimates \rho_1$ and $\hat{\rho}_0  \estimates \rho_0$ when $g$ is ideal. When $g$ is not ideal, to our knowledge perfect estimation of $\rho_1$ and $\rho_0$ is impossible and at best \textbf{Goal 1} is to provide exact expressions for $\hat{\rho}_1$ and $\hat{\rho}_0$ w.r.t. $\rho_1$ and $\rho_0$. \textbf{Goal 2} is to use $\hat{\rho}_1$ and $\hat{\rho}_0$ to uncover the classifications of $f$ from $g$. Both tasks must be accomplished given only observed ($x,s$) pairs. $y, \rho_1, \rho_0, \pi_1$, and $\pi_0$ are hidden.

% In terms of these conditions, \textbf{Goal 1} is to find an algorithm for perfect estimation of $\rho_1$ and $\rho_0$ when $g$ is ideal. When $g$ is not ideal, to our knowledge perfect estimation of $\rho_1$ and $\rho_0$ is impossible 
% %when we allow $g$ to be imperfect due to random added noise or $P$ and $N$ have overlapping support without restriction. Thus, when $g$ is non-ideal, 
% and at best \textbf{Goal 1} is to provide exact expressions for $\hat{\rho_1}$ and $\hat{\rho_0}$ and their relations to $\rho_1$ and $\rho_0$. \textbf{Goal 2} is unchanged. 
% % To achieve this, we prove that the expected risk for the modified loss induced by Rank Pruning is equivalent to the expected risk of the underlying perfectly labeled dataset.

==> uai_rp_arxiv copy/0_intro.tex <==

\section{Introduction}
\label{sec:intro}

Consider a student with no knowledge of animals tasked with learning to classify whether a picture contains a dog. A teacher shows the student example pictures of lone four-legged animals, stating whether the image contains a dog or not. Unfortunately, the teacher may often make mistakes, asymmetrically, with a significantly large false positive rate, $\rho_1 \in [0,1]$, and significantly large false negative rate, $\rho_0 \in [0,1]$. The teacher may also include ``white noise" images with a uniformly random label. This information is unknown to the student, who only knows of the images and corrupted labels, but suspects that the teacher may make mistakes. Can the student (1) estimate the mistake rates, $\rho_1$ and $\rho_0$, (2) learn to classify pictures with dogs accurately, and (3) do so efficiently (e.g. less than an hour for 50 images)? This allegory clarifies the challenges of $\tilde{P}\tilde{N}$ learning for any classifier trained with corrupted labels, perhaps with intermixed noise examples. We elect the notation $\tilde{P}\tilde{N}$ to emphasize that both the positive and negative sets may contain mislabeled examples, reserving $P$ and $N$ for uncorrupted sets.

This example illustrates a fundamental reliance of supervised learning on training labels \citep{Michalski:1986:MLA:21934}. Traditional learning performance degrades monotonically with label noise \citep{Aha1991, Nettleton2010}, necessitating semi-supervised approaches \citep{Blanchard:2010:SND:1756006.1953028}. Examples of noisy datasets are medical \citep{raviv_heart}, human-labeled \citep{mech_turk_quality}, and sensor \citep{lane2010survey} datasets. The problem of uncovering the same classifications as if the data was not mislabeled is our fundamental goal.

Towards this goal, we introduce Rank Pruning\footnote{ Rank Pruning is open-source and available at \href{http://bit.ly/2pbtjR6}{https://github.com/cgnorthcutt/rankpruning}}, an algorithm for $\tilde{P}\tilde{N}$ learning composed of two sequential parts: (1) estimation of the asymmetric noise rates $\rho_1$ and $\rho_0$ and (2) removal of mislabeled examples prior to training. The fundamental mantra of Rank Pruning is \emph{learning with confident examples}, i.e. examples with a predicted probability of being positive \emph{near} $1$ when the label is positive or $0$ when the label is negative. If we imagine non-confident examples as a noise class, separate from the confident positive and negative classes, then their removal should unveil a subset of the uncorrupted data. 

An ancillary mantra of Rank Pruning is \emph{removal by rank} which elegantly exploits ranking without sorting. Instead of pruning non-confident examples by predicted probability, we estimate the number of mislabeled examples in each class. We then remove the $k^{th}$-most or $k^{th}$-least examples, \emph{ranked} by predicted probability, via the BFPRT algorithm \citep{Blum:1973:TBS:1739940.1740109} in $\mathcal{O}(n)$ time, where $n$ is the number of training examples. \emph{Removal by rank} mitigates sensitivity to probability estimation and exploits the reduced complexity of learning to rank over probability estimation \citep{Menon2012PredictingAP}. Together, \emph{learning with confident examples} and \emph{removal by rank} enable robustness, i.e. invariance to erroneous input deviation.

% In essence, confident examples are those having agreement of predicted probability and training label. If an example has a positive label, but a low predicted probability of being positive, we prune out this training example from the dataset. The intuition is that non-confident examples are likely to be mislabeled and their removal may unveil a subset of the true, uncorrupted distribution. If so, then the expected risk of training on the pruned set is equivalent to training on the correctly labeled data. 

Beyond prediction, confident examples help estimate $\rho_1$ and $\rho_0$. Typical approaches require averaging predicted probabilities on a holdout set \citep{Liu:2016:CNL:2914183.2914328, Elkan:2008:LCO:1401890.1401920} tying noise estimation to the accuracy of the predicted probabilities, which in practice may be confounded by added noise or poor model selection. Instead, we estimate $\rho_1$ and $\rho_0$ as a fraction of the predicted counts of confident examples in each class, encouraging robustness for variation in probability estimation.


\subsection{Related Work}

% Rank Pruning bridges framework, nomenclature, and application across three areas of semi-supervised learning: (1) one-class classification and $PU$ learning, (2) $\tilde{P}\tilde{N}$ learning, and (3) domain adaptation. In this section, we consider the contributions of Rank Pruning in the context of each.

% Rank Pruning bridges framework, nomenclature, and application across three areas of semi-supervised learning: (1) one-class classification, (2) $PU$ learning, and (3) $\tilde{P}\tilde{N}$ learning. In this section, we consider the contributions of Rank Pruning in the context of each.

Rank Pruning bridges framework, nomenclature, and application across $PU$ and $\tilde{P}\tilde{N}$ learning. In this section, we consider the contributions of Rank Pruning in both.

% \subsubsection{One-class Classification \& \texorpdfstring{$PU$}{PU} Learning}
\subsubsection{\texorpdfstring{$PU$}{PU} Learning}

% One-class classification \citep{moya_1993_oneclass} is distinguished from binary classification by a training set containing examples from only one class, making it useful for outlier and novelty detection \citep{ Hempstalk:2008:oneclass}. This can be framed as $\tilde{P}\tilde{N}$ learning when outliers take the form of mislabeled examples. The predominant approach, one-class SVM, fits a hyper-boundary around the training class \citep{oneclasssvm1999}, but often performs poorly due to boundary over-sensitivity \citep{Manevitz:2002:OSD:944790.944808} and fails when the training class contains mislabeled examples.

Positive-unlabeled ($PU$) learning is a binary classification task in which a subset of positive training examples are labeled, and the rest are unlabeled. For example, co-training \citep{Blum:1998:CLU:279943.279962, Nigam00understandingthe} with labeled and unlabeled examples can be framed as a $PU$ learning problem by assigning all unlabeled examples the label `0'. $PU$ learning methods often assume corrupted negative labels for the unlabeled examples $U$ such that $PU$ learning is $\tilde{P}\tilde{N}$ learning with no mislabeled examples in $P$, hence their naming conventions.

Early approaches to $PU$ learning modified the loss functions via weighted logistic regression \citep{lee2003PUlearning_weightedlogreg} and biased SVM \citep{Liu:2003:BTC:951949.952139} to penalize more when positive examples are predicted incorrectly. Bagging SVM \citep{Mordelet:2014:BSL:2565612.2565683} and RESVM \citep{Claesen201573} extended biased SVM to instead use an ensemble of classifiers trained by resampling $U$ (and $P$ for RESVM) to improve robustness \citep{Breiman:1996:BP:231986.231989}. RESVM claims state-of-the-art for $PU$ learning, but is impractically inefficient for large datasets because it requires optimization of five parameters and suffers from the pitfalls of SVM model selection \citep{Chapelle:1999:MSS:3009657.3009690}. \cite{Elkan:2008:LCO:1401890.1401920} introduce a formative time-efficient probabilistic approach (denoted \emph{Elk08}) for $PU$ learning that directly estimates $1 - \rho_1$ by averaging predicted probabilities of a holdout set and dividing all predicted probabilities by $1 - \rho_1$. On the SwissProt database, \emph{Elk08} was 621 times faster than biased SVM, which only requires two parameter optimization. However, \emph{Elk08} noise rate estimation is sensitive to inexact probability estimation and both RESVM and \emph{Elk08} assume $P$ = $\tilde{P}$ and do not generalize to $\tilde{P}\tilde{N}$ learning.  Rank Pruning leverages \emph{Elk08} to initialize $\rho_1$, but then re-estimates $\rho_1$ using confident examples for both robustness (RESVM) and efficiency (\emph{Elk08}).

% Early approaches to $PU$ learning modified the loss functions of weighted logistic regression \citep{lee2003PUlearning_weightedlogreg} and biased SVM \citep{Liu:2003:BTC:951949.952139} to penalize more when positive examples are predicted incorrectly. Bagging SVM \citep{Mordelet:2014:BSL:2565612.2565683} extended biased SVM to instead use an ensemble of classifiers trained by resampling $U$ to improve robustness \citep{Breiman:1996:BP:231986.231989}, arguing that biased SVM suffers from classifier instability due to the corrupted unlabeled set. RESVM \citep{Claesen201573} extended bagging SVM by additional resampling of $P$ to increase variability between base models. RESVM claims to be the current state-of-the-art for $PU$ learning.

% Unfortunately, RESVM is impractically inefficient for large datasets because it requires optimization of five parameters and suffers from the pitfalls of model selection for SVM \citep{Chapelle:1999:MSS:3009657.3009690}. A good paper by \cite{Elkan:2008:LCO:1401890.1401920} introduces an efficient probabilistic approach to PU learning that directly estimates the complementary noise rate $1 - \rho_1$ by averaging predicted probabilities on a holdout set and then dividing the predicted probabilities by $1 - \rho_1$. We abbreviate this method as \emph{Elk08}. For a classification task on the SwissProt database, \emph{Elk08} was 621 times faster than biased SVM, which only requires two parameter optimization. However, \emph{Elk08} noise rate estimation is highly sensitive to probability estimation which may be poor when the noise rate is large. Additionally, because \emph{Elk08} assumes $P$ is perfectly labeled, it performs poorly in the general $\tilde{P}\tilde{N}$ learning setting.  Rank Pruning leverages \emph{Elk08} to initialize $\rho_1$, but then re-estimates $\rho_1$ using confident examples for both robustness (RESVM) and efficiency (\emph{Elk08}).


\begin{table*}[t]
\caption{Variable definitions and descriptions for $\tilde{P}\tilde{N}$ learning and  PU learning. Related work contains a prominent author using each variable. $\rho_1$ is also referred to as \emph{contamination} in PU learning literature.}
 \vskip -0.15in
\label{t:definitions}
\begin{center}
\begin{small}
\begin{sc}

\resizebox{\textwidth}{!}{
\begin{tabular}{lcccr}
\toprule
\abovestrut{0.13in}\belowstrut{0.05in}
\textbf{Variable} & \textbf{Conditional} & \textbf{Description} & \textbf{Domain} & \textbf{Related} Work \\
\midrule
\abovestrut{0.1in}

$\rho_0$ & $P(s=1|y=0)$ & Fraction of $N$ examples mislabeled as positive & $\tilde{P}\tilde{N}$ & Liu \\
$\rho_1$ & $P(s=0|y=1)$ & Fraction of $P$ examples mislabeled as negative & $\tilde{P}\tilde{N}$, PU & Liu, Claesen \\
$\pi_0$ & $P(y=1|s=0)$ & Fraction of mislabeled examples in $\tilde{N}$ & $\tilde{P}\tilde{N}$ & Scott \\
$\pi_1$ & $P(y=0|s=1)$ & Fraction of mislabeled examples in $\tilde{P}$ & $\tilde{P}\tilde{N}$ & Scott \\
$c = 1- \rho_1$ & $P(s=1|y=1)$ & Fraction of correctly labeled $P$ if $P(y=1|s=1) = 1$ & PU & Elkan \\
% $\hat{\rho}^{prob}_1$ & $P(\hat{s}=0|s=1)$ & Predicted label inconsistency for examples in $\tilde{P}$ & $\tilde{P}\tilde{N}$ & Elkan \\
% $\hat{\rho}^{prob}_0$ & $P(\hat{s}=1|s=0)$ & Predicted label inconsistency for examples in $\tilde{N}$ & $\tilde{P}\tilde{N}$ &  \\

\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
 \vskip -0.25in
\end{table*}

\begin{table*}[b]
\renewcommand{\arraystretch}{.5}% Makes table rows tighter
\caption{Summary of state-of-the-art and selected general solutions to $\tilde{P}\tilde{N}$ and $PU$ learning.}
\vskip -.17in
\label{t:related_works}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
\abovestrut{0.05in}\belowstrut{0.05in}
\textbf{Related Work} & \textbf{Noise} & \textbf{$\tilde{P}\tilde{N}$} & \textbf{$PU$} & \textbf{Any Prob.} & \textbf{Prob Estim.} &                                     \textbf{Time}         & \textbf{Theory} & \textbf{Added} \\
                      & \textbf{Estim.} &                               &               & \textbf{Classifier} & \textbf{Robustness} &               \textbf{Efficient} & \textbf{Support} & \textbf{Noise} \\
\midrule
\abovestrut{0.1in}

\cite{Elkan:2008:LCO:1401890.1401920} & \checkmark &            & \checkmark & \checkmark &            & \checkmark & \checkmark & \\
\midrule
\cite{Claesen201573} &            &            & \checkmark &            & \checkmark &            &   &         \\
\midrule
\cite{ScottBH13} & \checkmark &            &            & \checkmark & \checkmark &            & \checkmark &\\
\midrule
\cite{NIPS2013_5073} &            & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark &\\
\midrule
\cite{Liu:2016:CNL:2914183.2914328} &            & \checkmark & \checkmark & \checkmark &            & \checkmark & \checkmark &\\
\midrule
\midrule
\textbf{Rank Pruning} & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\

\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
%  \vskip -0.25in
\end{table*}

\subsubsection{\texorpdfstring{$\tilde{P}\tilde{N}$}{Noisy PN} Learning}

Theoretical approaches for $\tilde{P}\tilde{N}$ learning often have two steps: (1) estimate the noise rates, $\rho_1$, $\rho_0$, and (2) use $\rho_1$, $\rho_0$ for prediction. To our knowledge, Rank Pruning is the only time-efficient solution for the open problem \mbox{\citep{Liu:2016:CNL:2914183.2914328, ICML2012Yang_127}} of noise estimation.

We first consider relevant work in noise rate estimation. \cite{ScottBH13} established a lower bound method for estimating the \emph{inversed} noise rates $\pi_1$ and $\pi_0$ (defined in Table \ref{t:definitions}). However, the method can be intractable due to unbounded convergence and assumes that the positive and negative distributions are mutually irreducible. Under additional assumptions, \cite{scott2015rate} proposed a time-efficient method for noise rate estimation, but reported poor performance \cite{Liu:2016:CNL:2914183.2914328}. \cite{Liu:2016:CNL:2914183.2914328} used the minimum predicted probabilities as the noise rates, which often yields futile estimates of min = $0$. \cite{NIPS2013_5073} provide no method for estimation and view the noise rates as parameters optimized with cross-validation, inducing a sacrificial accuracy, efficiency trade-off. In comparison, Rank Pruning noise rate estimation is time-efficient, consistent in ideal conditions, and robust to imperfect probability estimation.

\cite{NIPS2013_5073} developed two methods for prediction in the $\tilde{P}\tilde{N}$ setting which modify the loss function. The first method constructs an unbiased estimator of the loss function for the true distribution from the noisy distribution, but the estimator may be non-convex even if the original loss function is convex. If the classifier's loss function cannot be modified directly, this method requires splitting each example in two with class-conditional weights and ensuring split examples are in the same batch during optimization. For these reasons, we instead compare Rank Pruning with their second method (\emph{Nat13}), which constructs a label-dependent loss function such that for 0-1 loss, the minimizers of \emph{Nat13}'s risk and the risk for the true distribution are equivalent. 

%Given any convex and class-calibrated surrogate loss function, the label-dependent loss is also convex.

\cite{Liu:2016:CNL:2914183.2914328} generalized \emph{Elk08} to the $\tilde{P}\tilde{N}$ learning setting by modifying the loss function with per-example importance reweighting (\emph{Liu16}), but reweighting terms are derived from predicted probabilities which may be sensitive to inexact estimation. To mitigate sensitivity, \cite{Liu:2016:CNL:2914183.2914328} examine the use of density ratio estimation \citep{Sugiyama:2012:DRE:2181148}. Instead, Rank Pruning mitigates sensitivity by learning from confident examples selected by rank order, not predicted probability. For fairness of comparison across methods, we compare Rank Pruning with their probability-based approach. 


Assuming perfect estimation of $\rho_1$ and $\rho_0$, we, \cite{NIPS2013_5073}, and \cite{Liu:2016:CNL:2914183.2914328} all prove that the expected risk for the modified loss function is equivalent to the expected risk for the perfectly labeled dataset. However, both \cite{NIPS2013_5073} and \cite{Liu:2016:CNL:2914183.2914328} effectively "flip" example labels in the construction of their loss function, providing no benefit for added random noise. In comparison, Rank Pruning will also remove added random noise because noise drawn from a third distribution is unlikely to appear confidently positive or negative. Table \ref{t:related_works} summarizes our comparison of $\tilde{P}\tilde{N}$ and $PU$ learning methods.

% Liu assumes perfect probability estimation, whereas Rank Pruning weakly assumes range separability, defined in the next two sections. Natarajan makes no assumption and proves that the empirical risk of their first method is an upper bound for the expected risk. 
%Keeping in mind the ``no free lunch" theorem, 
% Given that all three methods show risk equivalence for , we might expect them to perform similarly. However, 

Procedural efforts have improved robustness to mislabeling in the context of machine vision \citep{Xiao2015LearningFM}, neural networks \citep{noisy_boostrapping_google}, and face recognition \citep{angelova2005pruning}. Though promising, these methods are restricted in theoretical justification and generality, motivating the need for Rank Pruning.

% % GREAT CNN PARAGRAPH BELOW, SHOULD ADD IF POSSIBLE

% Efforts to improve robustness to mislabeling in the context of machine vision \citep{Xiao2015LearningFM} use the term ``consistency" to capture the notion of confident examples. In a face recognition task with 90\% of non-faces mislabeled as faces, a bagging model combined with consistency voting was used to remove images with poor voting consistency \citep{angelova2005pruning}. In the context of deep learning, consistency of predictions from noisy training labels was enforced by combining a typical cross-entropy loss with an auto-encoder loss \citep{noisy_boostrapping_google}. This method enforces label consistency by constraining the network to uncover the input examples given the output prediction. Though promising, all of these methods are restricted in theoretical justification and generality, motivating the need for Rank Pruning.

% \subsubsection{Domain Adaptation}

% Domain adaptation is used in transfer learning to make predictions about a target distribution using a model learned from a related source distribution \citep{jiang2008literature}. This allows for robustness to outliers by uncovering noise in the source domain that cannot be adapted \citep{Chang:2012:RVD:2354409.2355115}. Domain adaptation has also been used to overcome label noise in object recognition via noisy existing human labels \citep{xu2016webly}. $\tilde{P}\tilde{N}$ learning can be re-framed as domain adaptation by considering the noisy labels as the source distribution and the hidden true labels as the target distribution. 

\subsection{Contributions}

In this paper, we describe the Rank Pruning algorithm for binary classification with imperfectly labeled training data. In particular, we:

\vskip -0.05in
\begin{itemize}
\vskip -0.05in
\itemsep.05in 
        \item Develop a robust, time-efficient, general solution for both $\tilde{P}\tilde{N}$ learning, i.e. binary classification with noisy labels, and estimation of the fraction of mislabeling in both the positive and negative training sets.
        \item Introduce the \emph{learning with confident examples} mantra as a new way to think about robust classification and estimation with mislabeled training data.
        \item Prove that under assumptions, Rank Pruning achieves perfect noise estimation and equivalent expected risk as learning with correct labels. We provide closed-form solutions when those assumptions are relaxed.
        \item Demonstrate that Rank Pruning performance generalizes across the number of training examples, feature dimension, fraction of mislabeling, and fraction of added noise examples drawn from a third distribution.
        \item Improve the state-of-the-art of $\tilde{P}\tilde{N}$ learning across F1 score, AUC-PR, and Error. In many cases, Rank Pruning achieves nearly the same F1 score as learning with correct labels when 50\% of positive examples are mislabeled and 50\% of observed positive labels are mislabeled negative examples.
    \end{itemize}


















==> uai_rp_arxiv copy/0_method.tex <==

\section{Rank Pruning}\label{methodology}

We develop the Rank Pruning algorithm to address our two goals. In Section \ref{method:noise}, we propose a method for noise rate estimation and prove consistency when $g$ is ideal. An estimator is ``consistent" if it achieves perfect estimation in the expectation of infinite examples. In Section \ref{method:noise_non_ideal}, we derive exact expressions for $\hat{\rho}_1$ and $\hat{\rho}_0$ when $g$ is unassuming. In Section \ref{method:rp}, we provide the entire algorithm, and in Section \ref{method:risk}, prove that Rank Pruning has equivalent expected risk as learning with uncorrupted labels for both ideal $g$ and non-ideal $g$ with weaker assumptions. Throughout, we assume $n \rightarrow \infty$ so that $P$ and $N$ are the hidden distributions, each with infinite examples. This is a necessary condition for Theorems. \ref{thm:noise_ideal}, \ref{rho_conf_robust} and Lemmas \ref{thm:lemma1}, \ref{lemma3}.


\subsection{Deriving Noise Rate Estimators \texorpdfstring{$\hat{\rho}_1^{conf}$ and $\hat{\rho}_0^{conf}$}{}} \label{method:noise}


We propose the \emph{confident counts} estimators $\hat{\rho}_1^{conf}$ and $\hat{\rho}_0^{conf}$ to estimate $\rho_1$ and $\rho_0$ as a fraction of the predicted counts of confident examples in each class, encouraging robustness for variation in probability estimation. To estimate $\rho_1=P(s=0|y=1)$, we count the number of examples with label $s=0$ that we are ``confident" have label $y=1$ and divide it by the total number of examples that we are ``confident" have label $y = 1$. More formally, 

\vskip -0.2in
\begin{equation}\label{define_rho_conf}
\hat{\rho}_1^{conf}:=\frac{|\tilde{N}_{y=1}|}{|\tilde{N}_{y=1}|+|\tilde{P}_{y=1}|}, \qquad
\hat{\rho}_0^{conf}:=\frac{|\tilde{P}_{y=0}|}{|\tilde{P}_{y=0}|+|\tilde{N}_{y=0}|}
\end{equation}
\vskip -0.1in

such that

\vskip -0.05in
\begin{equation}\label{define_threshold}
\begin{cases}
\tilde{P}_{y=1}=\{x\in\tilde{P}\mid g(x)\geq LB_{y=1}\}\\
\tilde{N}_{y=1}=\{x\in\tilde{N}\mid g(x)\geq LB_{y=1}\}\\
\tilde{P}_{y=0}=\{x\in\tilde{P}\mid g(x)\leq UB_{y=0}\}\\
\tilde{N}_{y=0}=\{x\in\tilde{N}\mid g(x)\leq UB_{y=0}\}
\end{cases}
\end{equation}
\vskip -0.1in

where $g$ is fit to the corrupted training set $D_{\rho}$ to obtain $g(x)=P(\hat{s}=1|x)$. The threshold $LB_{y=1}$ is the predicted probability in $g(x)$ above which we guess that an example $x$ has hidden label $y = 1$, and similarly for upper bound $UB_{y=0}$. $LB_{y=1}$ and $UB_{y=0}$ partition $\tilde{P}$ and $\tilde{N}$ into four sets representing a \emph{best guess} of a \emph{subset} of examples having labels (1) $s=1, y=0$, (2) $s=1, y=1$, (3) $s=0, y=0$, (4) $s=0, y=1$. The threshold values are defined as

\vskip -0.15in
\begin{equation*}
\begin{cases}
LB_{y=1}:=P(\hat{s}=1\mid s=1)=E_{x\in\tilde{P}}[g(x)]\\
UB_{y=0}:=P(\hat{s}=1\mid s=0)=E_{x\in\tilde{N}}[g(x)]\\
\end{cases}
\end{equation*}
\vskip -0.1in

where $\hat{s}$ is the predicted label from a classifier fit to the observed data. $|\tilde{P}_{y=1}|$ counts examples with label $s=1$ that are \emph{most} likely to be correctly labeled ($y=1$) because $LB_{y=1} = P(\hat{s}=1|s=1)$. The three other terms in Eq. (\ref{define_threshold}) follow similar reasoning. Importantly, the four terms do not sum to $n$, i.e. $|N| + |P|$, but $\hat{\rho}_1^{conf}$ and $\hat{\rho}_0^{conf}$ are valid estimates because mislabeling noise is assumed to be uniformly random. 
%If noise is perfectly uniform and $g$ range separates $P$ and $N$, then any thresholds $LB_{y=1}$ and $UB_{y=0}$ would yield the same counts in Eq. (\ref{define_threshold}). 
The choice of threshold values relies on the following two important equations:

\vskip -0.25in
\begin{align*}
LB_{y=1}=&E_{x\in\tilde{P}}[g(x)]=E_{x\in\tilde{P}}[P(s=1|x)]\\
=&E_{x\in\tilde{P}}[P(s=1|x,y=1)P(y=1|x)+P(s=1|x,y=0)P(y=0|x)]\\
=&E_{x\in\tilde{P}}[P(s=1|y=1)P(y=1|x)+P(s=1|y=0)P(y=0|x)]\\
=&(1-\rho_1)(1-\pi_1)+\rho_0\pi_1\numberthis \label{rh1_prob_eq}
\end{align*}
\vskip -0.05in

Similarly, we have

\vskip -0.15in
\begin{equation}\label{rh0_prob_eq}
UB_{y=0}=(1-\rho_1)\pi_0+\rho_0(1-\pi_0)
\end{equation}
\vskip -0.05in


To our knowledge, although simple, this is the first time that the relationship in Eq. (\ref{rh1_prob_eq}) (\ref{rh0_prob_eq}) has been published, linking the work of \cite{Elkan:2008:LCO:1401890.1401920}, \cite{Liu:2016:CNL:2914183.2914328}, \cite{ScottBH13} and \cite{NIPS2013_5073}. From Eq. (\ref{rh1_prob_eq}) (\ref{rh0_prob_eq}), we observe that $LB_{y=1}$ and $UB_{y=0}$ are linear interpolations of $1-\rho_1$ and $\rho_0$ and since $\rho_0 < 1- \rho_1$, we have that $\rho_0 < LB_{y=1} \leq 1-\rho_1$ and $\rho_0 \leq UB_{y=0} < 1-\rho_1$. When $g$ is ideal we have that $g(x)=(1-\rho_1)$, if $x \in P$ and $g(x)=\rho_0$, if $x \in N$. Thus  when $g$ is ideal, the thresholds $LB_{y=1}$ and  $UB_{y=0}$ in Eq. (\ref{define_threshold}) will perfectly separate $P$ and $N$ examples within each of $\tilde{P}$ and $\tilde{N}$. Lemma \ref{thm:lemma1} immediately follows.


\begin{lemma}\label{thm:lemma1}
\vskip -.1in
When $g$ is ideal,
\vskip -0.25in

\begin{align*}
\tilde{P}_{y=1} &= \{x\in P\mid s=1\},
\tilde{N}_{y=1} = \{x\in P\mid s=0\},\\
\tilde{P}_{y=0} &= \{x\in N\mid s=1\},
\tilde{N}_{y=0} = \{x\in N\mid s=0\}\numberthis
\end{align*}
\vskip -0.3in
\end{lemma}
\vskip -0.15in

Thus, when $g$ is ideal, the thresholds in Eq. (\ref{define_threshold}) partition the training set such that $\tilde{P}_{y=1}$ and $\tilde{N}_{y=0}$ contain the correctly labeled examples and $\tilde{P}_{y=0}$ and $\tilde{N}_{y=1}$ contain the mislabeled examples. Theorem \ref{thm:noise_ideal} follows (for brevity, proofs of all theorems/lemmas are in Appendix \ref{sec:A1}-\ref{sec:A5}).


\begin{theorem} \label{thm:noise_ideal}

When $g$ is ideal,
\vskip -0.15in
\begin{equation}
\hat{\rho}_1^{conf}=\rho_1, \hat{\rho}_0^{conf}=\rho_0
\end{equation}
\end{theorem}


Thus, when $g$ is ideal, the \emph{confident counts} estimators $\hat{\rho}_1^{conf}$ and $\hat{\rho}_0^{conf}$ are consistent estimators for $\rho_1$ and $\rho_0$ and we set $\hat{\rho}_1:=\hat{\rho}_1^{conf}, \hat{\rho}_0:=\hat{\rho}_0^{conf}$. These steps comprise Rank Pruning noise rate estimation (see Alg. \ref{alg:rp}). There are two practical observations. First, for any $g$ with $T$ fitting time, computing $\hat{\rho}_1^{conf}$ and $\hat{\rho}_0^{conf}$ is $\mathcal{O}(T)$. Second, $\hat{\rho}_1$ and $\hat{\rho}_0$ should be estimated out-of-sample to avoid over-fitting, resulting in sample variations. In our experiments, we use 3-fold cross-validation, requiring at most $2T=\mathcal{O}(T)$. 

\subsection{Noise Estimation: Unassuming Case} \label{method:noise_non_ideal}
 
Theorem \ref{thm:noise_ideal} states that $\hat{\rho}_i^{conf} = \rho_i$, $\forall i \in \{0,1\}$ when $g$ is ideal. Though theoretically constructive, in practice this is unlikely. Next, we derive expressions for the estimators when $g$ is unassuming, i.e. $g$ may not be perfect and $P$ and $N$ may have overlapping support.

Define $\Delta p_o:=\frac{|P \cap N|}{|P \cup N|}$ as the fraction of overlapping examples in $\mathcal{D}$ and remember that $\Delta g(x) := g(x)-g^*(x)$. Denote $ LB_{y=1}^*=(1-\rho_1)(1-\pi_1)+\rho_0\pi_1, UB_{y=0}^*=(1-\rho_1)\pi_0+\rho_0(1-\pi_0)$. We have

\begin{lemma}\label{lemma3}
When $g$ is unassuming, we have

\vskip -0.1in
\begin{equation}\label{rho_imperfect_condition}
\begin{cases}
LB_{y=1}=LB_{y=1}^*+E_{x\in\tilde{P}}[\Delta g(x)]-\frac{(1-\rho_1-\rho_0)^2}{p_{s1}}\Delta p_o\\
UB_{y=0}=UB_{y=0}^*+E_{x\in\tilde{N}}[\Delta g(x)]+\frac{(1-\rho_1-\rho_0)^2}{1-p_{s1}}\Delta p_o\\
\hat{\rho}_1^{conf}=\rho_1+\frac{1-\rho_1-\rho_0}{|P|-|\Delta P_1| + |\Delta N_1|}|\Delta N_1|\\
\hat{\rho}_0^{conf}=\rho_0+\frac{1-\rho_1-\rho_0}{|N|-|\Delta N_0| + |\Delta P_0|}|\Delta P_0|
\end{cases}
\end{equation}
\vskip -0.1in



where

\vskip -0.15in
\begin{equation*}
\begin{cases}
\Delta P_1=\{x\in P\mid g(x)< LB_{y=1}\}\\
\Delta N_1=\{x\in N\mid g(x)\geq LB_{y=1}\}\\
\Delta P_0=\{x\in P\mid g(x)\leq UB_{y=0}\}\\
\Delta N_0=\{x\in N\mid g(x)> UB_{y=0}\}\\
\end{cases}
\end{equation*}
\vskip -0.35in
\end{lemma}
\vskip -0.1in

The second term on the R.H.S. of the $\hat{\rho}_i^{conf}$ expressions captures the deviation of $\hat{\rho}_i^{conf}$ from $\rho_i$, $i=0,1$. This term results from both imperfect $g(x)$ and overlapping support. Because the term is non-negative, $\hat{\rho}_i^{conf} \geq \rho_i$, $i=0,1$ in the limit of infinite examples. In other words, $\hat{\rho}_i^{conf}$ is an \emph{upper bound} for the noise rates $\rho_i$, $i=0,1$. From Lemma \ref{lemma3}, it also follows:

\begin{theorem}\label{rho_conf_robust}
Given non-overlapping support condition,

\text{If} $\forall x\in N, \Delta g(x)<LB_{y=1}-\rho_0$, then $\hat{\rho}_1^{conf}=\rho_1$.

If $\forall x\in P, \Delta g(x)>-(1-\rho_1-UB_{y=0}$), then $\hat{\rho}_0^{conf}=\rho_0$.
\end{theorem}

Theorem \ref{rho_conf_robust} shows that $\hat{\rho}_1^{conf}$ and $\hat{\rho}_0^{conf}$ are robust to imperfect probability estimation. As long as $\Delta g(x)$ does not exceed the distance between the threshold in Eq. (\ref{define_threshold}) and the perfect $g^*(x)$ value, $\hat{\rho}_1^{conf}$ and $\hat{\rho}_0^{conf}$ are consistent estimators for $\rho_1$ and $\rho_0$. Our numerical experiments in Section \ref{sec:experimental} suggest this is reasonable for $\Delta g(x)$. The average $|\Delta g(x)|$ for the MNIST training dataset across different ($\rho_1$, $\pi_1$) varies between 0.01 and 0.08 for a logistic regression classifier, 0.01$\sim$0.03 for a CNN classifier, and 0.05$\sim$0.10 for the CIFAR dataset with a CNN classifier. Thus, when  $LB_{y=1}-\rho_0$ and $1-\rho_1-UB_{y=0}$ are above 0.1 for these datasets, from Theorem  \ref{rho_conf_robust} we see that $\hat{\rho}_i^{conf}$ still accurately estimates $\rho_i$.


\subsection{The Rank Pruning Algorithm} \label{method:rp}

Using $\hat{\rho}_1$ and $\hat{\rho}_0$, we must uncover the classifications of $f$ from $g$. In this section, we describe how Rank Pruning selects confident examples, removes the rest, and trains on the pruned set using a reweighted loss function. 

First, we obtain the inverse noise rates $\hat{\pi}_1$, $\hat{\pi}_0$ from $\hat{\rho}_1$, $\hat{\rho}_0$:

\vskip -0.13in
\begin{equation}
\hat{\pi}_1=\frac{\hat{\rho}_0}{p_{s1}}\frac{1-p_{s1}-\hat{\rho}_1}{1-\hat{\rho}_1-\hat{\rho}_0},\qquad
\hat{\pi}_0=\frac{\hat{\rho}_1}{1-p_{s1}}\frac{p_{s1}-\hat{\rho}_0}{1-\hat{\rho}_1-\hat{\rho}_0}
\end{equation}
\vskip -0.07in


Next, we prune the $\hat{\pi}_1|\tilde{P}|$ examples in $\tilde{P}$ with smallest $g(x)$ and the $\hat{\pi}_0|\tilde{N}|$ examples in $\tilde{N}$ with highest $g(x)$ and denote the pruned sets $\tilde{P}_{conf}$ and $\tilde{N}_{conf}$. To prune, we define $k_1$ as the $(\hat{\pi}_1|\tilde{P}|)^{th}$ smallest $g(x)$ for $x \in \tilde{P}$ and $k_0$ as the $(\hat{\pi}_0|\tilde{N}|)^{th}$ largest $g(x)$ for $x \in \tilde{N}$. BFPRT ($\mathcal{O}(n)$) \citep{Blum:1973:TBS:1739940.1740109} is used to compute $k_1$ and $k_0$ and pruning is reduced to the following $\mathcal{O}(n)$ filter:

\vskip -0.13in
\begin{equation}
\tilde{P}_{conf} := \{x \in \tilde{P} \mid g(x) \geq k_1 \},\qquad 
\tilde{N}_{conf} := \{x \in \tilde{N} \mid g(x) \leq k_0 \}
\end{equation}
\vskip -0.05in



Lastly, we refit the classifier to $X_{conf} = \tilde{P}_{conf} \cup \tilde{N}_{conf}$ by class-conditionally reweighting the loss function for examples in $\tilde{P}_{conf}$ with weight $\frac{1}{1-\hat{\rho}_1}$ and examples in $\tilde{N}_{conf}$ with weight $\frac{1}{1-\hat{\rho}_0}$ to recover the estimated balance of positive and negative examples. The entire Rank Pruning algorithm is presented in Alg. \ref{alg:rp} and illustrated step-by-step on a synthetic dataset in Fig. \ref{rankpruning_illustration}.

We conclude this section with a formal discussion of the loss function and efficiency of Rank Pruning.  Define $\hat{y_i}$ as the predicted label of example $i$ for the classifier fit to $X_{conf}, s_{conf}$ and let $l(\hat{y_i}, s_i)$ be the original loss function for $x_i \in D_\rho$. Then the loss function for Rank Pruning is simply the original loss function exerted on the pruned $X_{conf}$, with class-conditional weighting:


\vskip -0.25in
\begin{align*}  \label{rank_pruning_loss_function}
\tilde{l}(\hat{y_i}, s_i)=&\frac{1}{1-\hat{\rho}_1}l(\hat{y_i}, s_i)\cdot\indicator{x_i\in \tilde{P}_{conf}}+ \frac{1}{1-\hat{\rho}_0}l(\hat{y_i}, s_i)\cdot\indicator{x_i\in \tilde{N}_{conf}}\numberthis 
\end{align*}

\medskip

Effectively this loss function uses a zero-weight for pruned examples. Other than potentially fewer examples, the only difference in the loss function for Rank Pruning and the original loss function is the class-conditional weights. These constant factors do not increase the complexity of the minimization of the original loss function. In other words, we can fairly report the running time of Rank Pruning in terms of the running time ($\mathcal{O}(T)$) of the choice of probabilistic estimator. Combining noise estimation ($\mathcal{O}(T)$), pruning ($\mathcal{O}(n)$), and the final fitting ($\mathcal{O}(T)$), Rank Pruning has a running time of $\mathcal{O}(T) + \mathcal{O}(n)$, which is $\mathcal{O}(T)$ for typical classifiers.


\subsection{Rank Pruning: A simple summary}

Recognizing that formalization can create obfuscation, in this section we describe the entire algorithm in a few sentences. Rank Pruning takes as input training examples $X$, noisy labels $s$, and a probabilistic classifier $clf$ and finds a subset of $X, s$ that is likely to be correctly labeled, i.e. a subset of $X, y$. To do this, we first find two thresholds, $LB_{y=1}$ and $UB_{y=0}$, to \emph{confidently} guess the correctly and incorrectly labeled examples in each of $\tilde{P}$ and $\tilde{N}$, forming four sets, then use the set sizes to estimate the noise rates $\rho_1 = P(s = 0 | y = 1)$ and $\rho_0 = P(s = 1 | y = 0)$. We then use the noise rates to estimate the number of examples with observed label $s = 1$ and hidden label $y = 0$ and remove that number of examples from $\tilde{P}$ by removing those with lowest predicted probability $g(x)$. We prune $\tilde{N}$ similarly. Finally, the classifier is fit to the pruned set, which is intended to represent a subset of the correctly labeled data.

\begin{algorithm}[t]
   \caption{\textbf{Rank Pruning}}
   \label{alg:rp}
\begin{algorithmic}
   \STATE {\bfseries Input:} Examples $X$, corrupted labels $s$, classifier clf
   \STATE \textbf{Part 1. Estimating Noise Rates:}
   \STATE (1.1)\ \ clf.fit($X$,$s$)
   \STATE \ \ \ \ \ \ \ \ \ $g(x)\leftarrow$clf.predict\_crossval\_probability($\hat{s}=1|x$)
   \STATE \ \ \ \ \ \  \ \ \ $p_{s1}=\frac{\text{count}(s=1)}{\text{count}(s=0 \lor s=1)}$
   \STATE \ \ \ \ \ \  \ \ \ $LB_{y=1}=E_{x\in\tilde{P}}[g(x)]$, $UB_{y=0}=E_{x\in\tilde{N}}[g(x)]$
   \STATE (1.2)\  $\hat{\rho}_1=\hat{\rho}_1^{conf}=\frac{|\tilde{N}_{y=1}|}{|\tilde{N}_{y=1}|+|\tilde{P}_{y=1}|}$, $\hat{\rho}_0=\hat{\rho}_0^{conf}=\frac{|\tilde{P}_{y=0}|}{|\tilde{P}_{y=0}|+|\tilde{N}_{y=0}|}$
   \STATE \ \ \ \ \ \ \ \ \ $\hat{\pi}_1=\frac{\hat{\rho}_0}{p_{s1}}\frac{1-p_{s1}-\hat{\rho}_1}{1-\hat{\rho}_1-\hat{\rho}_0}$, $\hat{\pi}_0=\frac{\hat{\rho}_1}{1-p_{s1}}\frac{p_{s1}-\hat{\rho}_0}{1-\hat{\rho}_1-\hat{\rho}_0}$
   \vskip .1in
   \STATE \textbf{Part 2. Prune Inconsistent Examples:}
   \STATE (2.1) Remove $\hat{\pi}_1|\tilde{P}|$ examples in $\tilde{P}$ with least $g(x)$, Remove $\hat{\pi}_0|\tilde{N}|$ examples in $\tilde{N}$ with greatest $g(x)$,
   \STATE \ \ \ \ \ \ \ \ \ Denote the remaining training set ($X_{conf}$, $s_{conf}$)
   \STATE (2.2) clf.fit($X_{conf}$, $s_{conf}$), with sample weight 
   $w(x)=\frac{1}{1-\hat{\rho}_1}\indicator{s_{conf}=1}$+$\frac{1}{1-\hat{\rho}_0}\indicator{s_{conf}=0}$
   \STATE {\bfseries Output:} clf
\end{algorithmic}
\end{algorithm}

\subsection{Expected Risk Evaluation} 
\label{method:risk}

In this section, we prove Rank Pruning exactly uncovers the classifier $f$ fit to hidden $y$ labels when $g$ range separates $P$ and $N$ and $\rho_1$ and $\rho_0$ are given.

Denote $f_{\theta}\in\mathcal{F}: x\to \hat{y}$ as a classifier's prediction function belonging to some function space $\mathcal{F}$, where $\theta$ represents the classifier's parameters. $f_{\theta}$ represents $f$, but without $\theta$ necessarily fit to the training data. $\hat{f}$ is the Rank Pruning estimate of $f$.

% Denote the empirical risk of $f_{\theta}$ w.r.t. the loss function $l$ and distribution $\mathcal{D}$ as $\hat{R}_{l,\mathcal{D}}(f_{\theta})=\frac{1}{n}\sum_{i=1}^n\tilde{l}(f_{\theta}(x_i), s_i)$, and the expected risk $R_{l,\mathcal{D}}(f_{\theta})=E_{(x,y)\sim \mathcal{D}}[\hat{R}_{l,\mathcal{D}}(f_{\theta})]$. We show that using Rank Pruning, a classifier $\hat{f}$ can be learned for the hidden data $(X, y)$, given the corrupted data $(X, s)$, by minimizing the empirical risk $\hat{R}_{\tilde{l},D_{\rho}}(f_{\theta})$:

Denote the empirical risk of $f_{\theta}$ w.r.t. the loss function $\tilde{l}$ and corrupted data $D_{\rho}$ as $\hat{R}_{\tilde{l}, D_{\rho}}(f_{\theta})=\frac{1}{n}\sum_{i=1}^n\tilde{l}(f_{\theta}(x_i), s_i)$, and the expected risk of $f_{\theta}$ w.r.t. the corrupted distribution $\mathcal{D}_{\rho}$ as $R_{\tilde{l},\mathcal{D}_{\rho}}(f_{\theta})=E_{(x,s)\sim \mathcal{D}_{\rho}}[\hat{R}_{\tilde{l},\mathcal{D}_{\rho}}(f_{\theta})]$. Similarly, denote $R_{l,\mathcal{D}}(f_{\theta})$ as the expected risk of $f_{\theta}$ w.r.t. the hidden distribution $\mathcal{D}$ and loss function $l$. We show that using Rank Pruning, a classifier $\hat{f}$ can be learned for the hidden data $D$, given the corrupted data $D_{\rho}$, by minimizing the empirical risk:

\vskip -0.12in
\begin{equation}\label{risk_minimization}
\hat{f}=\argmin\limits_{f_{\theta}\in \mathcal{F}} \hat{R}_{\tilde{l},D_{\rho}}(f_{\theta})=\argmin\limits_{f_{\theta}\in \mathcal{F}} \frac{1}{n}\sum_{i=1}^n\tilde{l}(f_{\theta}(x_i), s_i)
\end{equation}

Under the \emph{range separability} condition, we have

\begin{figure}[t]
\begin{center}
\centerline{\includegraphics[width=1.0\columnwidth]{rankpruning_illustration_horizontal.pdf}}
\caption{Illustration of Rank Pruning with a logistic regression classifier ($\mathcal{LR}_\theta$).  \textbf{(a)}: The corrupted training set $D_\rho$ with noise rates $\rho_1=0.4$ and $\rho_0=0.1$. Corrupted colored labels (\textcolor{blue}{$s=1$},\textcolor{red}{$s=0$}) are observed. $y$ ($+$,$-$) is hidden. \textbf{(b)}: The marginal distribution of $D_\rho$ projected onto the $x_p$ axis (indicated in (a)), and the $\mathcal{LR}_\theta$'s estimated $g(x)$, from which $\hat{\rho}_1^{conf}=0.4237$, $\hat{\rho}_0^{conf}=0.1144$ are estimated. \textbf{(c)}: The pruned $X_{conf}, s_{conf}$. \textbf{(d)}: The classification result by Rank Pruning ($\hat{f}$ = $\mathcal{LR}_\theta.\text{fit}(X_{conf}, s_{conf})$),
ground truth classifier ($f$ = $\mathcal{LR}_\theta.\text{fit}(X,y)$),
and baseline classifier ($g$ = $\mathcal{LR}_\theta.\text{fit}(X, s)$), with an accuracy of $94.16\%$, $94.16\%$ and $78.83\%$, respectively.}
\label{rankpruning_illustration}
\end{center}
\vskip -0.15in
\end{figure}

\begin{theorem}\label{Rank Pruning_with_range_separability}
If $g$ range separates $P$ and $N$ and $\hat{\rho}_i=\rho_i$, $i=0,1$, then for any classifier $f_{\theta}$ and any bounded loss function $l(\hat{y}_i,y_i)$, we have

\vskip -0.12in
\begin{equation}
R_{\tilde{l},\mathcal{D}_{\rho}}(f_{\theta})=R_{l,\mathcal{D}}(f_{\theta})
\end{equation}
\vskip -0.06in


where $\tilde{l}(\hat{y}_i,s_i)$ is Rank Pruning's loss function (Eq. \ref{rank_pruning_loss_function}).
\end{theorem}



The proof of Theorem \ref{Rank Pruning_with_range_separability} is in Appendix \ref{sec:A5}. Intuitively, Theorem \ref{Rank Pruning_with_range_separability} tells us that if $g$ range separates $P$ and $N$, then given exact noise rate estimates, Rank Pruning will exactly prune out the positive examples in $\tilde{N}$ and negative examples in $\tilde{P}$, leading to the same expected risk as learning from uncorrupted labels. Thus, Rank Pruning can exactly uncover the classifications of $f$ (with infinite examples) because the expected risk is equivalent for any $f_{\theta}$. Note Theorem \ref{Rank Pruning_with_range_separability} also holds when $g$ is ideal, since \emph{ideal} $\subset$ \emph{range separability}. In practice, \emph{range separability} encompasses a wide range of imperfect $g(x)$ scenarios, e.g. $g(x)$ can have large fluctuation in both $P$ and $N$ or have systematic drift w.r.t. to $g^*(x)$ due to underfitting. 

% When $g$ does not range separate $P$ and $N$, Rank Pruning is still invariant to imperfect $g(x)$ within a range separable subset of $P$ and $N$. Because Rank Pruning uses confident examples for robustness, when noise rate estimates are inexact, Rank Pruning maintains comparatively superior performance as shown in our experiments in the next section.
